Picking Apart Story Salads

During natural disasters and conflicts, information about what happened is often confusing, messy, and distributed across many sources. We would like to be able to automatically identify relevant information and assemble it into coherent narratives of what happened. To make this task accessible to neural models, we introduce Story Salads, mixtures of multiple documents that can be generated at scale. By exploiting the Wikipedia hierarchy, we can generate salads that exhibit challenging inference problems. Story salads give rise to a novel, challenging clustering task, where the objective is to group sentences from the same narratives. We demonstrate that simple bag-of-words similarity clustering falls short on this task and that it is necessary to take into account global context and coherence.

==> _05-experiments.tex <==
\section{Experiments \& Results}
\label{sec:experiments}

\textbf{Configuration}. All the experiments described in this section use the \s{nyt} dataset (Section \ref{sec:data}), with a vocabulary cut of top 100k. For evaluation we randomly sample 1k mixtures from the test set\footnote{List of exact test items used will be made available upon acceptance.}, and report the average score over 20 samples. For the baselines \s{km} and \s{hac} we use the default configurations\footnote{\s{km}: \burl{github.com/letiantian/kmedoids}; \\\s{hac}: \burl{scipy.cluster.hierarchy}.} of off-the-shelf software. All the neural components are constructed with \texttt{Tensorflow} and use the same hyperparameters across variants: 2-layered BiLSTM, learning rate 1e-5, dropout \cite{Srivastava:14} rate 0.3, Xavier initialization \cite{Glorot:10}. To create training sentence pairs for the neural classifiers, we evenly and randomly sample $[A,A], [A,B], [B,A]$, and $[B,B]$ pairs, $\{A,B\}$ being the pseudo labels for the narratives. Sampling 8 pairs for each pairing configuration we come to a batch size of 32. Finally, all the models are run until a stopping condition is met: less than 1e-5 accuracy improvement on the validation set, which is 5\% of mixtures sampled from the training data. 
\smallskip

\noindent
\textbf{Evaluation}. We evaluate all models uniformly with one metric. We adopt a simple \emph{clustering accuracy} metric (hereafter \textsc{ca}): 
we calculate the ratio of correctly clustered sentences in a document mixture, averaged over test mixtures.
%calculating the ratio of correctly clustered sentences in a document mixture, and taking the average \textsc{ca} over the evaluated subset.
%As the cluster labels do not carry meaning, we create two labels $\{A,B\}$ for our binary setup. For a document mixture $d_i$, which has $N_i$ sentences, we compute the following:
Given a document mixture $d_i$, we call its component documents $A$ and $B$. Let \texttt{pred} be a function that does the clustering by mapping each sentence $s_{i,n}$ of mixture $d_i$ to either 0 or 1. Then the clustering accuracy for document $d_i$ by \texttt{pred} is

{\small\begin{align*}
\textsc{ca}(d_i, \texttt{pred}) &= \texttt{max}\{\textsc{c}(d_i;\langle A,B\rangle),\textsc{c}(d_i;\langle B,A\rangle)\}\\
\textsc{c}(d_i) &= \frac{1}{N_i}\sum_{n=1}^{N_i} \mathds{1}[L(\texttt{pred}(s_{i,n})) = \texttt{true}(s_{i,n})]
\end{align*}}
%where \s{c} is a cluster label assignment, $s_{i,n}$ is the $n$-th sentence in $d_i$, and $\texttt{pred}(s_{i,n}) = \texttt{true}(s_{i,n})$ indicates the sentence $s_{i,n}$ belong to the same cluster both in the predicted and the true partition, $\langle A,B\rangle$ and $\langle B,A\rangle$ are the two ways of labeling the clusters. 

\noindent
where $L$ is a cluster label assignment that either maps 0 to $A$ and 1 to $B$, or the other way round, and $s_{i,n}$ is the $n$-th sentence of mixture $d_i$.
Doing so we avoid issues with overestimation working with a binary clustering task
%\footnote{Our clustering task is nonstandard in that we assume the knowledge of the number of clusters. Thus the frequently used clustering metrics do not apply well in our setting and tend to overestimate model performances.} 
\cite{im-Walde:03}.
\smallskip

\begin{comment}
\begin{table}[!t]
\begin{center}
\scalebox{0.80}{
\begin{tabular}{lcc}
\toprule
Model & \textsc{cls-a} & \textsc{ca} \\
\midrule
\s{unif} & -- & 52.7 \\
\s{km} (average embedding) & -- & 76.4 \\
\midrule
\textsc{bilstm} & 81.7 & 78.5 \\
\textsc{bilstm-mt} & 82.6 & 80.8 \\
\textsc{bilstm-context} & 84.4 & 82.6 \\
\textsc{bilstm-mt-context} & \textbf{87.3} & \textbf{84.9} \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Results summary for baselines and neural classifier aided clustering. \textsc{cls-a}: classification accuracy; \textsc{ca}: clustering accuracy. \s{km} with average embedding is the best-performing baseline, the classifier aided clusterers are therefore all based on it.}
\label{tab:base-bilstm}
\end{table}
\end{comment}

\begin{table}[!t]
\begin{center}
\scalebox{0.80}{
\begin{tabular}{lc}
\toprule
Model & \textsc{nyt}-test \\
\midrule
\s{unif} & 52.7 \\
\s{km} (average embedding) & 76.4 \\
\midrule
\textsc{bilstm} & 78.5 \\
\textsc{bilstm-mt} & 80.8 \\
\textsc{bilstm-context} & 82.6 \\
\textsc{bilstm-mt-context} & \textbf{84.9} \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Results summary for baselines and neural classifier aided clustering. The scores reported are clustering accuracy. \s{km} with average embedding is the best-performing baseline, the classifier aided clusterers are therefore all based on it.}
\label{tab:base-bilstm}
\end{table}

\noindent
\textbf{Experiments}. We start out by running \s{unif} baseline, which produces 52.7 accuracy, indicating that our data is more or less balanced in the number of sentences in the two narratives of mixtures. 
%Next, we run the two common baseline clustering algorithms (i.e. \s{km} and \s{hac}) with three sentence embedding methods discussed above (i.e. average word embedding, skip-thought and SCDV).
We first compare the baselines to the neural classifier-clusterer variants. The results are shown in Table \ref{tab:base-bilstm}.
The best model emerges from the experiments is \s{km} with average word embedding at 76.4 in clustering accuracy. In general \s{km}-based models are $\sim$2 points better than \s{hac}, and average word embedding based models are over 10 points above skip-thought and SCDV based models. 
\smallskip

\noindent
We then augment the best performing clustering algorithm (i.e. \s{km}) with our four variants of BiLSTM-based neural classifier\footnote{We experimented with various hidden sizes for LSTM cells and found little difference across dimensions from 75D to 200D. We thus choose the best performing 100D setup.}: \s{bilstm}, \s{bilstm-mt}, \s{bilstm-ctx}, and \s{bilstm-mt-ctx}. We observe that (i) all the classifier aided \s{km}s perform better than the base \s{km} (the best model is at 84.9, which is 8.5 points higher than \s{km} in accuracy); (ii) both mutual attention and context reading boost improve performance on the base \s{bilstm}, and the contributions are to a large extent orthogonal, which is indicated by the fact that the combined model (\s{bilstm-mt-ctx}) outperform single-component augmented models (\s{bilstm-mt}, \s{bilstm-ctx}). 
%The results of the all the experiments above are summarized in Table \ref{tab:base-bilstm}. 
\smallskip

\begin{table}[!t]
\begin{center}
\scalebox{0.80}{
\begin{tabular}{lccc}
\toprule
Model & \s{nyt-hard} & \s{wiki-hard} & \s{wiki}-test \\
\midrule
\s{km} & 59.8 & 60.4 & 71.9 \\
\midrule
\s{bilstm} & 55.3 & 57.9 & 72.4 \\
\s{bilstm-mt} & 56.7 & 58.5 & 74.0 \\
\s{bilstm-ctx} & 63.8 & 63.3 & 74.6 \\
\s{bilstm-mt-ctx} & \textbf{68.0} & \textbf{64.2} & \textbf{76.7} \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Results summary for experiment on top 1k sample by topic similarity (\s{tsim}): \s{nyt-hard} and \s{wiki-hard} and the test set of \s{wiki} dataset. The scores reported are clustering accuracy.}
\label{tab:tsim-ood}
\end{table}

\noindent
Next we explore the generality of our models. First, note that mixtures are not equally difficult to cluster: the ones that are topically similar (e.g. where two narratives in a mixture are both on business, sports or military conflict) are intuitively much more difficult to cluster for models that rely on vocabulary similarity/overlapping. This applies to our baseline \s{km} clusterer and classifier aided \s{bilstm-km}. This type of mixtures is important because in many practical scenario we would expect to see topically similar mixtures. E.g. the conflicting reports an investigative journalist expect to sort by narrative. To explore, we apply a simple \emph{topic similarity} score (\bs{tsim}) to sample 1k mixtures from the test set of both \s{nyt} (call it \s{nyt-hard}) and \s{wiki-hard} and see how our models do on this sample: the \s{tsim} of a mixture is the cosine similarity between the average word embeddings of its two narratives:
\begin{equation}
\s{tsim}(d) = \texttt{cosine}(g(\omega_1), g(\omega_2))
\end{equation}
where $\omega_1, \omega_2$ are the two narratives in $d$, each is a set of sentences, $g$ is a shorthand for the function that computes the average embeddings of the narratives' constituent words (i.e. words from all sentences in a narrative). The average \s{tsim} of \s{nyt-hard} and \s{wiki-hard} are 0.56 and 0.64 respectively. The performance of all our models plummets on the two difficult samples, with the best performing \s{bilstm-mt-ctx} only manages to yield 68.0 \s{nyt-hard} and 64.2 on \s{wiki-hard}. 
\smallskip

\noindent
Second, we believe that a reasonable expectation with the \emph{story salads} task is being able to train a general-purpose model on a large body of text and use it in a to some extent out-of-domain scenario. That is, we want to see if we could use the models to learn ``meta knowledge'' about clustering document mixtures. To investigate, we apply the same protocol (averaging over 20 1k-mixture samples from test set) to evaluate out-of-domain on \s{wiki}-test. In terms of difficulty as measured by \s{tsim} score, \s{nyt} and \s{wiki} are roughly in the same ballpark, at 0.33 and 0.35 respectively. These experiments are summarized in Table \ref{tab:tsim-ood}.
\smallskip

\begin{table}[!t]
\begin{center}
\scalebox{0.75}{
\begin{tabular}{lcc}
\toprule
Model & \s{nyt-event}-test & \s{nyt-event-hard} \\
\midrule
\s{km} & 64.7 & 55.3 \\
\midrule
\s{ffnn-bilstm-base} & 64.9 & 54.8 \\
\s{ffnn-bilstm} & 66.8 & 59.1 \\
\s{ffnn-pi-bilstm} & \textbf{70.2} & \textbf{61.4} \\
\s{rf-pi-bilstm} & 68.3 & 60.5 \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Results summary for event-based models. \s{nyt-event}-test: the test set of the event version of \s{nyt}. \s{nyt-event-hard}: the 1k top topically similar mixtures are sampled from \s{nyt-event}-test. The scores reported are clustering accuracy.}
\label{tab:event}
\end{table}

\noindent
Finally we experiment with the \s{nyt-event} dataset with our event-based models, which are based on our strongest BiLSTM classifier (i.e. \s{bilstm-mt-ctx}). As for the sentence-based experiments, we sample 1k most topically similar mixtures for an additional experiment (call it \s{nyt-event-hard}). As before we run \s{km} as the baseline. The results from the event-based experiment are much lower than the sentence-based, on average over 10 points below. The best-performing is \s{ffnn-pi-bilstm}, which reports 70.2 clustering accuracy. Regardless, the classifier aided models clear a good margin above the baseline \s{km}. On the topically most similar mixtures, as before, we observe the same pattern that all models take a massive hit in accuracy. Finally the results from \s{ffnn-bilstm-base} confirms that mutual attention and contextualization are effective as in the sentence-based experiments. The results of the event-based experiments are summarized in Table \ref{tab:event}. 
\smallskip





%The results are summarized in Table \ref{tab:exp-4}. Here we see a dramatic overall reduction in performance, consistent with our intuition that mixtures with high \s{tsim} are more difficult for our models. More interestingly, we see that the mutual attention mechanism helps little, and the context reader becomes the main ``bread winner'' in improving performance upon the base \s{bilstm-km}, with the best model clearing 8.2 points above the \s{km} baseline.

\begin{comment}
\noindent
\textbf{Experiment 1}. For the first experiment we evaluate our baselines with the three sentence embedding methods discussed above. The results are reported in Table \ref{tab:exp-1}. Consistent with the findings of \citet{Coates:18}, we found empirical evidence that seemingly naive average word embeddings encoding scheme works surprisingly well. In fact, it outperforms more complex and sophisticated methods, i.e. skip-thought and SCDV, by a considerable margin.  
\smallskip

\begin{table}[!t]
\begin{center}
\scalebox{0.80}{
\begin{tabular}{lccc}
\toprule
Model & \multicolumn{3}{c}{\textsc{ca}} \\
\midrule
\textsc{unif} & \multicolumn{3}{c}{52.7} \\
\midrule
& Average embs. & skip-thought & SCDV \\
\midrule
\textsc{km} & \textbf{76.4} & 63.9 & 64.5 \\
\textsc{hac} & 74.4 & 61.5 & 63.0 \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Results from Experiment 1. \textsc{ca}: clustering accuracy. Two clustering algorithms are run with three variants on sentence embedding methods: average \texttt{GloVe}, skip-thought and SCDV.}
\label{tab:exp-1}
\end{table}

\noindent
\textbf{Experiment 2}. Next we evaluate our neural classifier-clusterer method. Based on the results from the previous experiment, for Experiment 2 we select \s{km} as our clustering algorithm and average \texttt{GloVe} embedding as the sentence embedding method. Specifically we compare the baseline \s{km} with \s{bilstm} aided \s{km} in various hidden sizes. The results are reported in Figure \ref{tab:exp-2}. We locate the ``sweet spot'' of 100D for the BiLSTM hidden size, and show that the classifier aided clusterer (\s{bilstm-km}) does perform better than the baseline clusterer, although only by a small margin. In addition, we see that the classification accuracy of the classifiers is well-aligned with the clustering accuracy. 
\smallskip

\begin{table}[!t]
\begin{center}
\scalebox{0.80}{
\begin{tabular}{lcc}
\toprule
Model & \textsc{cls-a} & \textsc{ca} \\
\midrule
\textsc{km} & -- & 76.4 \\
\midrule
\textsc{bilstm+km (75d)} & 80.6 & 77.5 \\
\textsc{bilstm+km (100d)} & \textbf{81.7} & \textbf{78.5} \\
\textsc{bilstm+km (200d)} & 80.4 & 77.1 \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Results from Experiment 2. \textsc{cls-a}: classification accuracy; \textsc{ca}: clustering accuracy. The BiLSTM aided \s{km} (\s{bilstm-km}) in various hidden sizes is pitched against the baseline \s{km}.}
\label{tab:exp-2}
\end{table}

\noindent
\textbf{Experiment 3}. To further gauge the difficulty of the \textsc{nyt} dataset, we incorporate the strong neural components described above --- mutual attention and context reader in this experiment. The results are reported in Table \ref{tab:exp-3}. Again the classification accuracy and clustering accuracy are well-aligned. Further we observe more or less orthogonal performance improvement by adding each neural component: the strongest \textsc{bilstm-mt-context+km} does better than the base BiLSTM and the base with only the mutual attention mechanism or the context reader. It clears a massive 8.5 points of accuracy over the \s{km} baseline.
\smallskip

\begin{table}[!t]
\begin{center}
\scalebox{0.80}{
\begin{tabular}{lcc}
\toprule
Model & \textsc{cls-a} & \textsc{ca} \\
\midrule
\textsc{bilstm+km} & 81.7 & 78.5 \\
\textsc{bilstm-mt+km} & 82.6 & 80.8 \\
\textsc{bilstm-context+km} & 84.4 & 82.6 \\
\textsc{bilstm-mt-context+km} & \textbf{87.3} & \textbf{84.9} \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Results from Experiment 3. \textsc{cls-a}: classification accuracy; \textsc{ca}: clustering accuracy. We report a complete ablation on the additional neural components to the base BiLSTM classifier (100D).}
\label{tab:exp-3}
\end{table}

\noindent
\textbf{Experiment 4}. Mixtures are not created equally. The ones that are topically similar (e.g. where two narratives in a mixture are both on business, sports or military conflict) are intuitively much more difficult to cluster for models that rely on vocabulary similarity/overlapping. This applies to our baseline \s{km} clusterer and classifier aided \s{bilstm-km}. This type of mixtures is important because in many practical scenario we would expect to see topically similar mixtures. E.g. the conflicting reports an investigative journalist expect to sort by narrative. To explore, we apply a simple \emph{topic similarity} score (\bs{tsim}) to sample 1k mixtures from the test set and see how our models do on this sample. The \s{tsim} of a mixture is the cosine similarity between the average word embeddings of its two narratives:
\begin{equation}
\s{tsim}(d) = \texttt{cosine}(g(\omega_1), g(\omega_2))
\end{equation}
where $\omega_1, \omega_2$ are the two narratives in $d$, each is a set of sentences, $g$ is a shorthand for the function that computes the average embeddings of the narratives' constituent words (i.e. words from all sentences in a narrative). The results are summarized in Table \ref{tab:exp-4}. Here we see a dramatic overall reduction in performance, consistent with our intuition that mixtures with high \s{tsim} are more difficult for our models. More interestingly, we see that the mutual attention mechanism helps little, and the context reader becomes the main ``bread winner'' in improving performance upon the base \s{bilstm-km}, with the best model clearing 8.2 points above the \s{km} baseline.
\smallskip

\begin{table}[!t]
\begin{center}
\scalebox{0.80}{
\begin{tabular}{lc}
\toprule
Model & \textsc{ca} \\
\midrule
\s{km} & 59.8 \\
\midrule
\textsc{bilstm+km} & 55.3 \\
\textsc{bilstm-mt+km} & 56.7 \\
\textsc{bilstm-context+km} & 63.8 \\
\textsc{bilstm-mt-context+km} & \textbf{68.0} \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Results from Experiment 4. \textsc{ca}: clustering accuracy. The models are evaluated on the top 1k topically most similar mixtures from the \s{nyt} test set.}
\label{tab:exp-4}
\end{table}

\noindent
\textbf{Experiment 5}. One reasonable expectation with the \emph{story salads} task is being able to train a general-purpose model on a large body of text and use it in a to some extent out-of-domain scenario. That is, we want to see if we could use the models to learn ``meta knowledge'' about disentangling document mixtures. In addition, like in Experiment 4, we want to gauge how well the models fare on more difficult mixtures. To investigate (and be consistent with how we evaluated on \s{nyt}), we evaluate the \s{nyt}-trained models on 20 (i) 1k random samples from the \s{wiki} set, and (i) 1k random samples from \s{wiki-hard} set. Computing \s{tsim} score for the two sample sets, we get 0.35 and 0.64 respectively, indicating that (ii) should be expected to be much harder. The results are reported in Table \ref{tab:exp-5}. The best score on \s{wiki} is lower than the in-domain \s{nyt}, but still holds a comfortable margin over the baseline. As expected, the performance plummets on the difficult set where \s{tsim} is high.
\smallskip

\begin{table}[!t]
\begin{center}
\scalebox{0.80}{
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{\textsc{ca}} \\
\cmidrule{2-3}
& \s{wiki} & \s{wiki-hard} \\
\midrule
\s{km} & 71.9 & 60.4 \\
\midrule
\textsc{bilstm+km} & 72.4 & 57.9 \\
\textsc{bilstm-mt+km} & 74.0 & 58.5 \\
\textsc{bilstm-context+km} & 74.6 & 63.3 \\
\textsc{bilstm-mt-context+km} & \textbf{76.7} & \textbf{64.2} \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Results from Experiment 5. \textsc{ca}: clustering accuracy. The average performance of our models evaluated on 20 1k samples from the out-of-domain \s{wiki} and \s{wiki-hard} sets.}
\label{tab:exp-5}
\end{table}

\end{comment}























































==> _06-analysis.tex <==
\section{Analysis}
\label{sec:analysis}

%\externaldocument{05-experiments}
%\ref{tab:baseline-bilstm}
%\pageref{tab:baseline-bilstm}

\noindent
\textbf{Overview}. First of all, we see from the first set of experiments (Table 3) that (i) the \emph{story salads} is a validly set up clustering task, in that our models learn to disentangle narratives in mixtures with reasonable effectiveness; (ii) classifier aided clustering does improve performance beyond a naive baseline (i.e. \s{km}), and adding additional neural component (i.e. mutual attention and context reader) produces strong clustering accuracy ($\sim$85\%) on easier mixtures (i.e. \s{nyt}) where humans can also easily perform the same task. Our models also generalize well in the out-of-domain setting (Table 4, \s{wiki}-test), where it's clear they do pick up on some form of ``meta knowledge'' which is universal to tackling \emph{story salads}. What this ``meta knowledge'' is motivates further work on the subject. 
\smallskip 

\begin{table}[!t]
\begin{center}
\scalebox{0.80}{
\begin{tabular}{llc}
\toprule
Type & Model & $\rho$(\s{ca},\s{tsim}) \\
\midrule
\multirow{2}{*}{-\s{context}} & \s{bilstm} & $-0.40^*$ \\
& \s{bilstm-mt} & $-0.38^*$ \\
\midrule
\multirow{2}{*}{+\s{context}} & \s{bilstm-ctx} & $-0.31^*$ \\
& \s{bilstm-mt-ctx} & $-0.27^*$ \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Spearman's $\rho$ correlation between clustering accuracy (\s{ca}) and topic similarity (\s{tsim}). The p-values are all below 0.01(*). Contextualized models (+\s{context}) are more robust to high topic similarity than their uncontextualized counterparts (-\s{context}).}
\label{tab:corr}
\end{table}

\noindent
On more challenging mixtures in subsequent experiments, i.e. where the topic similarity (\s{tsim}) between two narratives is high, and where the task is difficult even for humans, all the models suffer a substantial performance loss (Table 4, on \s{nyt-hard} and \s{wiki-hard}). 
Interestingly however, we see substantial improvement on these datasets when we add global context (i.e. mixture at hand) and mutual attention. We analyze this below qualitatively and quantitatively. 
%Because high \s{tsim} mixtures are of particular importance is the practical aspect of \emph{story salads} (recall the report-sorting task for our investigative journalist). \s{tsim} makes a good estimator of the difficulty of a mixture: quantitatively, \s{tsim} scores (negative) correlate strongly with clustering accuracy across models (Table \ref{tab:corr}). Qualitatively, the two narratives in mixtures with high \s{tsim} are often on the same topic (e.g. business, sports, or military conflict) and therefore tremendously hard to take apart even for a human agent \textcolor{red}{[Su] Examples below? But mixtures are gigantic and take a lot of space. Single-column is not an option.}.
\smallskip

\noindent
In event-based experiments (Table 5), we see that isolating out bare bone event tuples do not produce better performance. This shows that directly applying models developed on sentence-based data do not suffice: while it seems we've denoised the data by removing nonessential words, we may have lost the stylometric information contained therein the models rely on. Nevertheless, the results indicate that the event-based dataset provides a good opportunity for future modeling of coreference and narrative schema knowledge.

\begin{comment}
???In event-based experiments (Table 5), our hypothesis that the noise-less event-based data are easier to handle does not pan out: all the models plummet in performance. We suspect this to be due to our modeling choice: the models, while perform strong in the sentence-based data, do not take many sources of information available in event analysis, 
%in particular entity linking and coreference 
in particular coreference and narrative schema knowledge
--- essentially, compared to the sentence version, we only lose many words in the event version which could contain stylometric information which the models may depend on. Nevertheless, the results provide good motivation for future work where the value of these additional information sources can be fully explored.??? 
\end{comment}
\smallskip

\noindent
\textbf{Mutual attention and contextualization}. Across the board, the additional neural components prove to improve performance by a good margin. First we look at mutual attention. A base BiLSTM classifier encodes a sentence into a single vector (i.e. the final state), which is bound to lead to information loss \cite{Conneau:18}. Mutual attention allows us access to detailed information in sentences at word-level definition, which in particular captures lexical similarity. In fact, plotting heatmaps (Figure \ref{fig:mt-ctx-interaction}) of the attention weights, we see words/phrases that are distributionally similar are highlighted with higher weights. This distributional alignment, however as one would expect, is not effective on mixtures with topically similar narratives, where word overlapping is high (Table 4 on *\s{-hard} dataset), to which contextualization proves to be robust.
\smallskip

\noindent
The context reader is shown to be the most crucial performance improver for \emph{story salads}. Qualitatively, this highlights the distinctive aspect of the atypical clustering task: the contrast of two narratives is only meaningful \emph{in the context} of the particular mixture where they reside, rather than on a corpus-general level. Take the example in Table 1, the Russian-Chechnya and the U.S.-Afghanistan narratives are contrasted in that mixture, but one can easily imagine them being together as one narrative where a story on military conflict and one on business is contrasted in another mixture. Quantitatively, contextualized models are less vulnerable to the performance reduction on high-\s{tsim} mixtures: the negative correlation between accuracy and \s{tsim} is much lower in these models (Table \ref{tab:corr}). 
\smallskip

\begin{figure}[!t]
\begin{center}
\includegraphics[width=\linewidth]{FIGS/exp3-analysis-att-context.png}
\end{center}
\caption{Attention weight heatmaps for a random sample. Lighter color indicates higher attention weights. The two heatmaps in the same block are for the attention weights of one sentence attending to the other. In both (a) and (b), the left map is $s_1$ attending to $s_2$, the right map the other way around.}
\label{fig:mt-ctx-interaction}
\end{figure}

\noindent
Mutual attention also receives a positive boost when interacting with contextualization: in addition to distributionally similar words, it also sets high attention weights on phrases that are of contrastive value in-context. For example, in Figure \ref{fig:mt-ctx-interaction}, phrases like \emph{video game maker}, \emph{sega group}, which do not have distributionally similar words in the other sentence, come to have high weights (which is not the case without the context reader). 

\begin{table*}[!t]
\begin{center}
\scalebox{0.80}{
\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{On Plain \s{bilstm}} & \multicolumn{3}{c}{\s{bad}} & \multicolumn{3}{c}{\s{medium}} & \multicolumn{3}{c}{\s{good}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
& \s{b} & \s{m} & \s{g} & \s{b} & \s{m} & \s{g} & \s{b} & \s{m} & \s{g} \\
\midrule
+ Mutual Attention & 0.37 & 0.22 & 0.41 & 0.12 & 0.29 & 0.59 & 0.07 & 0.12 & 0.81 \\
+ Context & 0.37 & 0.30 & 0.33 & 0.12 & 0.35 & 0.53 & 0.06 & 0.19 & 0.75 \\
+ Both & 0.07 & 0.30 & 0.63 & 0.06 & 0.35 & 0.59 & 0.00 & 0.06 & 0.94 \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Sample study of model behavior on the same mixtures: the percentage of cases moved between performance brackets by adding component: $\s{bad} (\s{b}) = [0.5,0.65); \s{medium} (\s{m}) = [0.65,0.8); \s{good} (\s{g}) = [0.8,1.0]$. E.g. By adding Context, 33\% of the cases moved from \s{bad} to 
\s{good}. The pattern is clear that mutual attention and contextualization are capable of improving clustering accuracy at high probability.}
\label{tab:sample60-1}
\end{table*}

\begin{table}[!t]
\begin{center}
\scalebox{0.80}{
\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{On Plain \s{bilstm}} & \multicolumn{3}{c}{\s{bad}$\rightarrow$\s{good}} \\
\cmidrule{2-4}
& Distinct & Medium & Similar \\
\midrule
+ Mutual Attention & 0.55 & 0.27 & 0.18 \\
+ Context & 0.56 & 0.33 & 0.11 \\
+ Both & 0.41 & 0.12 & 0.47 \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Sample study of model behavior on the same mixtures: the percentage of cases moved between difficulty brackets by manual examination. ``Distinct'' being the easiest, ``Similar'' the hardest.}
\label{tab:sample60-2}
\end{table}

\noindent
Finally, we also probe the four model variants (i.e. plain, mutual attention only, context only, both. Table 3) in action on the same exact mixtures. Randomly taking 60 samples from \s{nyt}-test, we organize the results from the models in three bins by accuracy: $\s{bad} = [0.5,0.65); \s{medium} = [0.65,0.8); \s{good} = [0.8,1.0]$, and recorded the movement of the mixtures between bins across the models (Table \ref{tab:sample60-1}). Firstly, consistent with previous results (Table 3), mutual attention and contextualization help resolve the mixtures the plain model fails to handle. More interestingly, 
we see an interesting synergistic behavior: the combined model (i.e. in \s{bilstm-mt-ctx}) moves a much larger number of high-\s{tsim} mixtures from \s{bad} to \s{good} than the attention-only and context-only model (Table \ref{tab:sample60-2}). Specifically, we manually sort the mixtures into three difficulty brackets: (i) distinct: very easy to pick apart; (ii) medium: more difficult but still possible to pick apart; (iii) similar: very confusing and unable to pick apart. Here we see a high resolution rate of difficult mixtures by the combined model.
\smallskip

\noindent
\textbf{Challenges}. \textcolor{red}{[Su] Plan to summarize remaining challenges for story salads here. Any comments on what to included?}

%\noindent
%Across experiments, the mutual attention mechanism and contextualization improve 


\begin{comment}
\noindent
\bigskip
=== PREV. DRAFT BELOW ===
\bigskip

\noindent
\textbf{Sentence embedding}. We start by probing to understand how average embeddings would work better than more sophisticated methods. We suspect skip-thought is subject to strong performance deterioration as the length of encoded sentences gets longer. To investigate, we plot average sentence length in mixture against the clustering accuracy for the three types of embedding method (Figure \ref{fig:exp-1-analysis}). For SCDV, we conjecture it suffers from overfitting: a word embedding in SCDV is a large vector that is the concatenation of embeddings generated from all GMM components. We leave the investigation into this to future work.
\smallskip

\begin{figure}[!t]
\begin{center}
\includegraphics[width=60mm]{FIGS/exp1-analysis.png}
\end{center}
\caption{Plotting average sentence lengths against model performance in clustering accuracy. Embedding aggregation methods average embeddings and SCDV are not affected by longer sentences. Longer sentences contain more information for clustering for these methods. skip-thought on the other hand suffers with lengthier sentences.}
\label{fig:exp-1-analysis}
\end{figure}

\noindent
\textbf{Contextualization}. As we see in experiments 2 through 5, while the introduction of supervision with \s{bilstm-km} improve performance over the baseline \s{km} in most cases, by far the largest performance contributor has been the context reader. In particular, it manages to improve accuracy in tough tasks where mixtures are topically highly similar (Experiments 4, 5), where other variants are stuck below the baseline. Quantitatively, by computing the correlation between the \s{tsim} scores of mixtures and clustering accuracy, we find that contextualized models are more robust to topic similarity. The results are reported in Table \ref{tab:corr}. Qualitatively (\textcolor{red}{Example takes large space, how to get around?}).
\smallskip

\begin{table}[!t]
\begin{center}
\scalebox{0.80}{
\begin{tabular}{llc}
\toprule
Type & Model & $\rho$(\s{ca},\s{tsim}) \\
\midrule
\multirow{2}{*}{-\s{context}} & \s{bilstm+km} & $-0.40^*$ \\
& \s{bilstm-mt+km} & $-0.38^*$ \\
\midrule
\multirow{2}{*}{+\s{context}} & \s{bilstm-context+km} & $-0.31^*$ \\
& \s{bilstm-mt-context+km} & $-0.27^*$ \\
\bottomrule
\end{tabular}}
\end{center}
\caption{Spearman's $\rho$ correlation between clustering accuracy (\s{ca}) and topic similarity (\s{tsim}). The p-values are all below 0.01(*). Contextualized models (+\s{context}) are more robust to high topic similarity than their uncontextualized counterparts (-\s{context}).}
\label{tab:corr}
\end{table}

\noindent
\textbf{Mutual attention}. It is not surprising that mutual attention enhances performance: in the base \s{bilstm}, sentences are compressed into a single vector, and we lose information on individual words, which is particularly poignant with longer sentences. Mutual attention allows the model to look over individual word embeddings, thereby provides a better ``resolution''. Plotting heatmaps of attention weights of randomly sampled mixtures we see a nice alignment of distributionally similar words. Of more interest, however, is how the context reader helps mutual attention: contextually important words/phrases are attended to when context reader is included. For example, in Figure \ref{fig:exp-3-mt-context}, phrases like \emph{video game maker}, \emph{sega group}, which do not have distributionally similar words in the other sentence, come to have high attention weights (which is not the case without the context reader). This again highlights the importance of contextualization in \emph{story salads} as a nonstandard clustering task.

\begin{figure}[!t]
\begin{center}
\includegraphics[width=\linewidth]{FIGS/exp3-analysis-att-context.png}
\end{center}
\caption{Attention weight heatmpas for a random sample. Lighter color indicates higher attention weights. The two heatmaps in the same block are for the attention weights of one sentence attending to the other. Top block: two sentences from the same narrative; Bottom block: two sentences from different narratives.}
\label{fig:exp-3-mt-context}
\end{figure}

\end{comment}


































































